MedCLIPSeg: Probabilistic Vision-Language Adaptation for Data-Efficient and Generalizable Medical Image Segmentation

Medical image segmentation remains challenging due to limited annotations for training, ambiguous anatomical features, and domain shifts. While vision-language models such as CLIP offer strong cross-modal representations, their potential for dense, text-guided medical image segmentation remains underexplored. We present MedCLIPSeg, a novel framework that adapts CLIP for robust, data-efficient, and uncertainty-aware medical image segmentation. Our approach leverages patch-level CLIP embeddings through probabilistic cross-modal attention, enabling bidirectional interaction between image and text tokens and explicit modeling of predictive uncertainty. Together with a soft patch-level contrastive loss that encourages more nuanced semantic learning across diverse textual prompts, MedCLIPSeg effectively improves data efficiency and domain generalizability. Extensive experiments across 16 datasets spanning five imaging modalities and six organs demonstrate that MedCLIPSeg outperforms prior methods in accuracy, efficiency, and robustness, while providing interpretable uncertainty maps that highlight local reliability of segmentation results. This work demonstrates the potential of probabilistic vision-language modeling for text-driven medical image segmentation.

==> tables/hyperparameters.tex <==
\begin{table}[!htbp]
\centering
\caption{\small\textnormal{
Training hyperparameters for \texttt{MedCLIPSeg} across all datasets. }}
\tablestyle{-12pt}{1.1}
\addtolength{\tabcolsep}{+16pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l | c c c c c c c}
\toprule
\textbf{Dataset} & \textbf{Epochs} & \textbf{Batch Size} & \textbf{Learning Rate} & $\lambda_{\mathrm{Dice}}$ & $\lambda_{\mathrm{CE}}$ & $\lambda_{\mathrm{CLIP}}$ & $\beta$ \\
\midrule
BTMRI~\cite{Cheng2017} & 100 & 24 & $3\times10^{-4}$ & 0.5 & 0.5 & 0.1 & 2.35 \\
BUSI~\cite{busi} & 100 & 24 & $3\times10^{-4}$ & 0.5 & 0.5 & 0.1 & 2.35 \\
ISIC~\cite{isic1,isic2} & 100 & 24 & $3\times10^{-4}$ & 0.5 & 0.5 & 0.1 & 2.35 \\
Kvasir-Seg~\cite{jha2019kvasir} & 100 & 24 & $3\times10^{-4}$ & 0.5 & 0.5 & 0.1 & 2.35 \\
QaTa-COV19~\cite{qatacov19} & 100 & 24 & $3\times10^{-4}$ & 0.5 & 0.5 & 0.1 & 2.35 \\
EUS~\cite{jaramillo2020endoscopic} & 10 & 24 & $3\times10^{-4}$ & 0.5 & 0.5 & 0.1 & 2.35 \\
\bottomrule
\end{tabular}%
}
\label{tab:training_hyperparams}
\end{table}

==> tables/main_results_full.tex <==
\begin{table*}[t!]
\caption{\textbf{Fully supervised segmentation:} 
This table reports DSC and NSD values (\%) across six medical image segmentation benchmarks. 
All baseline methods are trained in a fully supervised manner using ground-truth annotations. Best results are in \textbf{bold}, and second-best are \underline{underlined}.}
\centering
\tablestyle{-27pt}{1.1}
\addtolength{\tabcolsep}{+30pt}
\renewcommand{\arraystretch}{1.5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{BUSI}} & \multicolumn{2}{c}{\textbf{BTMRI}}  & \multicolumn{2}{c}{\textbf{ISIC}} & \multicolumn{2}{c}{\textbf{Kvasir-Seg}} & \multicolumn{2}{c}{\textbf{QaTa-COV19}} & \multicolumn{2}{c}{\textbf{EUS}} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
& \textbf{DSC} $\uparrow$ & \textbf{NSD} $\uparrow$ & \textbf{DSC} $\uparrow$ & \textbf{NSD} $\uparrow$ & \textbf{DSC} $\uparrow$ & \textbf{NSD} $\uparrow$ & \textbf{DSC} $\uparrow$ & \textbf{NSD} $\uparrow$ & \textbf{DSC} $\uparrow$ & \textbf{NSD} $\uparrow$ 
& \textbf{DSC} $\uparrow$ & \textbf{NSD} $\uparrow$ \\ \midrule
\rowcolor{gray!15} \multicolumn{13}{c}{\texttt{\textbf{Unimodal Approaches}}} \\
UNet \cite{ronneberger2015unet}         & 70.04 & 73.88 & 86.06 & 90.71 & 89.10 & 92.06 & 80.26 & 83.53 & 76.97 & 82.32 & 68.53 & 69.92 \\
UNet++ \cite{zhou2018unet++}       & 67.54 & 71.15 & 83.30 & 87.94 & 89.36 & 92.17 & 84.81 & 88.07 & 73.52 & 78.23 & 72.08 & 73.15 \\
DeepLabv3 \cite{chen2017rethinking}    & 63.02 & 67.18 & 83.49 & 89.31 & 76.34 & 80.24 & 82.00 & 85.73 & 69.63 & 75.67 & 65.21 & 66.37 \\
AttnUNet \cite{oktay2018attention}     & 62.65 & 66.21 & 85.24 & 89.76 & 89.00 & 92.03 & 78.59 & 81.79 & 73.57 & 78.71 & 68.76 & 70.13 \\
nnUNet \cite{isensee2021nnu}       & 76.85 & 80.70 & \underline{86.91} & \underline{92.00} & 90.52 & \underline{93.37} & 85.44 & \underline{89.29} & 75.43 & 81.00 & 73.27 & 74.09 \\
Swin-UNet \cite{cao2022swin}  & 50.37 & 56.13 & 65.34 & 72.51 & 88.10 & 91.00 & 58.69 & 63.87 & 69.69 & 72.43 & 57.96 & 59.95 \\
TransUNet \cite{chen2021transunet} & 57.98 & 62.50 & 70.90 & 76.46 & 88.10 & 91.00 & 58.69 & 63.87 & 68.74 & 71.99 & 58.88 & 61.10 \\ \midrule
\rowcolor{gray!15}
\multicolumn{13}{c}{\texttt{\textbf{Generic Text-driven Approaches}}} \\
LAVT \cite{yang2022lavt} & 79.26 & 81.87 & 83.38 & 86.83 & 90.44 & 91.47 & 74.55 & 76.58 & 80.32 & 86.39 & 85.07 & 85.87 \\
LViT \cite{li2023lvit} & 75.32 & 77.99 & 81.41 & 84.80 & 91.21 & 92.22 & 85.29 & 87.30 & 82.31 & 87.80 & 84.53 & 85.23 \\ 
Ariadne's Thread \cite{zhong2023ariadne} & 57.26 & 58.22 & 69.96 & 71.40 & 68.37 & 69.30 & 77.42 & 78.79 & 70.70 & 73.94 & 76.71 & 77.31 \\ \midrule
\rowcolor{gray!15} \multicolumn{13}{c}{\texttt{\textbf{CLIP-Based Approaches}}} \\ 
CLIPSeg \cite{luddecke2022image} & \underline{80.95} & \underline{83.87} & 85.33 & 89.45 & 90.55 & 91.62 & 81.98 & 84.61 & 81.76 & 87.30 & 88.66 & 89.58 \\
DenseCLIP \cite{rao2022denseclip} & 71.85 & 74.39 & 70.30 & 72.34 & 89.29 & 90.32 & 79.32 & 81.37 & 65.84 & 72.72 & 68.52 & 70.17 \\ 
ZegCLIP \cite{zhou2023zegclip} & 72.08 & 74.45 & 76.65 & 79.77 & 81.45 & 82.33 & 78.46 & 80.43 & 75.42 & 82.59 & \underline{89.83} & \underline{90.54} \\
SAN \cite{xu2023side} & 77.99 & 80.75 & 85.27 & 89.14 & \underline{91.39} & 92.41 & 83.16 & 85.23 & 76.81 & 82.88 & 75.07 & 75.67 \\
MaPLe \cite{khattak2023maple} & 66.37 & 68.92 & 75.40 & 76.83 & 88.31 & 89.30 & 76.12 & 78.27 & 70.40 & 77.52 & 70.98 & 71.75 \\
MaPLe \cite{khattak2023maple} + Decoder & 80.49 & 83.38 & 85.08 & 89.20 & 90.10 & 91.21 & 83.46 & 85.96 & \underline{81.86} & \underline{88.16} & 88.65 & 89.55 \\
VLSM-Adapter \cite{dhakal2024vlsm} & 80.90 & 83.71 & 85.03 & 89.01 & 91.30 & 92.38 & \underline{85.89} & 88.34 & 81.15 & 87.10 & 78.82 & 79.76 \\
CausalCLIPSeg \cite{chen2024causalclipseg} & 76.11 & 78.70 & 81.71 & 85.30 & 89.47 & 90.46 & 78.77 & 80.79 & 75.67 & 82.37 & 86.30 & 87.59 \\  \midrule
\rowcolor{lightpurple}
\textbf{MedCLIPSeg (Ours)} & \textbf{85.33} & \textbf{88.00} & \textbf{88.15} & \textbf{92.06} & \textbf{92.30} & \textbf{93.36} & \textbf{89.65} & \textbf{91.81} & \textbf{84.07} & \textbf{89.79} & \textbf{91.59} & \textbf{92.39} \\
\bottomrule
\end{tabular}
}
\label{tab:main_results}
\end{table*}




